Be Your Own Neighborhood: Detecting Adversarial Example by the Neighborhood Relations Built on Self-Supervised Learning

Deep Neural Networks (DNNs) have achieved excellent performance in various fields. However, DNNs' vulnerability to Adversarial Examples (AE) hinders their deployments to safety-critical applications. This paper presents a novel AE detection framework, named BEYOND, for trustworthy predictions. BEYOND performs the detection by distinguishing the AE's abnormal relation with its augmented versions, i.e. neighbors, from two prospects: representation similarity and label consistency. An off-the-shelf Self-Supervised Learning (SSL) model is used to extract the representation and predict the label for its highly informative representation capacity compared to supervised learning models. For clean samples, their representations and predictions are closely consistent with their neighbors, whereas those of AEs differ greatly. Furthermore, we explain this observation and show that by leveraging this discrepancy BEYOND can effectively detect AEs. We develop a rigorous justification for the effectiveness of BEYOND. Furthermore, as a plug-and-play model, BEYOND can easily cooperate with the Adversarial Trained Classifier (ATC), achieving the state-of-the-art (SOTA) robustness accuracy. Experimental results show that BEYOND outperforms baselines by a large margin, especially under adaptive attacks. Empowered by the robust relation net built on SSL, we found that BEYOND outperforms baselines in terms of both detection ability and speed. Our code will be publicly available.

==> sections/4_theoretical_analysis.tex <==
\section{Robustness Analysis against Adaptive Attacks}
\label{sec:analysis}

% In this section, we analyze the effectiveness of our approach when the attacker is aware of our detection strategy.

\subsection{Adaptive Objective Loss Function}
\label{sec:design_ada}
Attackers can design adaptive attacks to bypass our detection when the attacker knows all the model parameters and detection strategy. To effectively attack \beyond, the adversary needs to deceive the target model while guaranteeing the label consistency and representation similarity of the SSL model. 
% To achieve the ultimate attack effect, we design the adaptive attack according to the suggestion of Croce et al. as follows:
Since \beyond uses multiple augmentations, we estimate the impact of all augmentations on label consistency and representation similarity during the attack as suggested by \cite{eval_robust}:
\begin{equation}
\begin{aligned}
    Sim_{l} &= \frac{1}{k} \sum_{i=1}^{k} \mathcal{L}\left(Cls\left(W_{aug}^i(x+\delta)  \right), y_t\right) \\
    Sim_{r} &= \frac{1}{k} \sum_{i=1}^{k}(\mathcal{S}(R(W_{aug}^i(x+\delta)), R(x+\delta))) \\
    % Loss_{ssl} & = Sim_l + \alpha Sim_{r} \\
\end{aligned}
\label{eq:analysis_1}
\end{equation}
where $\mathcal{S}$ represents the cosine similarity, and the adaptive adversaries perform gradient descent on the following combined objective:

\begin{equation}
    \underset{\delta}{min}~{\mathcal{L}_C(x+\delta, y_t) + Sim_l - Sim_{r}},
    \label{eq:adaptive}
\end{equation}
where $\mathcal{L}_C$ indicates classifier's loss function, and $y_t$ is the targeted class~\footnote{Note that we employ cosine metric is negatively correlated the similarity, so that the $Sim_{r}$ item is preceded by a minus sign.}.



% \subsection{Multi-objective Trade-off}
% % ensemble of models
% The above derivation shows that an attacker can mimic the SSL features of clean examples while misleading the target model. \beyond incorporates multiple data processing, which can be viewed as an ensemble of models. Each model shares parameters and applies different transformations to the inputs. Therefore, the attack must solve a multi-object optimization problem that deceives multiple models. However, it has been proven that creating adversarial images for multiple objects is fundamentally challenging~\cite{multitask}.

\subsection{Trade-off between label consistency and Representation Similarity}

Qualified adaptive attacks for \beyond are subject to the following conditions: misleading classifier while guaranteeing label consistency and representation similarity. For the classifier, its output for AEs is as follows:
\begin{equation}
\begin{aligned}    
    Cls(x+\delta)=& g(f(x+\delta)) \\
    \approx& g(f(x))+\nabla f(x) \frac{\partial g}{\partial f} \delta \\
    =& y + \nabla f(x) \frac{\partial g}{\partial f} \delta
\end{aligned}
\label{eq:analysis_3}
\end{equation}
Considering a single input transformation, label consistency can be formulated as the difference between the classifier's output of the AEs and their transformation:
\begin{equation}
\begin{aligned}    
    Sim_l =& g\left(f\left(W_{a u g} x+W_{a u g} \delta\right)\right)-g(f(x+\delta)) \\
    =& \nabla f(x) \frac{\partial g}{\partial f}\left(W_{a u g} \delta-\delta\right) \\
\end{aligned}
\label{eq:analysis_4}
\end{equation}

According to Eq. \ref{eq:analysis_3}, it can be seen that the optimization direction of the adaptive attack is the direction of increasing perturbation, which causes misclassification. However, the label consistency in Eq. \ref{eq:analysis_4} decreases when the perturbation increases. 
The empirical conclusion of Guo et al. shows that the input transformation can not weaken the perturbation when the perturbation is large enough ($W_{a u g}\delta = \delta$). Therefore, the optimization goal of the adversarial adaptive attack with high label consistency is to increase the perturbation.

According to Eq. \ref{eq:rs3} and Eq. \ref{eq:rs4}, the difference in representation similarity between adversarial samples and benign samples is expressed as follows:

\begin{equation}
\begin{aligned}    
    &R\left(W_{a u g} x_{a d v}\right) \odot R\left(x_{a d v}\right) - R(W_{a u g}x) \odot R(x) \\
    &= \nabla R(x)\delta \odot R(W_{a u g}x) \\
    &= \delta(\nabla R(x) \odot R(x))
\end{aligned}
\label{eq:analysis_5}
\end{equation}
\TODO{revise}
% \begin{equation}
% \begin{aligned}    
%     Sim_r =& R(W_{a u g}(x+\delta)) - R(x+\delta) \\
%     =& h\left(f\left(W_{a u g} x+W_{a u g} \delta\right)\right)-h(f(x+\delta))\\
%     =& f^{\prime}(x) \frac{\partial h}{\partial f}\left(W_{a u g} \delta-\delta\right)
% \end{aligned}
% \label{eq:analysis_5}
% \end{equation}
According to Eq. \ref{eq:analysis_5}, $R'(x) \odot R(x)$ is a constant, the difference in representation similarity between the AEs and benign samples is proportional to the perturbation, which must be as small as possible to ensure representation similarity. 

As a result, in case of the perturbation cannot bypass the transformation, the optimization direction of label consistency and representation similarity opposes, leading to the failure of the adaptive attack.
When the perturbation is large enough, although the adaptive attack can achieve good results, it also makes the adversarial perturbation more obvious, which is contrary to the imperceptibility of AEs.
% \pinyu{So what is our explanation againt Tramer's paper? He said detection is as difficult as robust classification, but we show detection is promising - why his conclusion won't apply to ours?}




